Whiz: A Fast and Flexible Data Analytics System

Today's data analytics frameworks are compute-centric, with analytics execution almost entirely dependent on the pre-determined physical structure of the high-level computation. Relegating intermediate data to a second class entity in this manner hurts flexibility, performance, and efficiency. We present Whiz, a new analytics framework that cleanly separates computation from intermediate data. It enables runtime visibility into data via programmable monitoring, and data-driven computation (where intermediate data values drive when/what computation runs) via an event abstraction. Experiments with a Whiz prototype on a large cluster using batch, streaming, and graph analytics workloads show that its performance is 1.3-2x better than state-of-the-art.

==> bib.tex <==
{ \footnotesize
   %\bibliographystyle{alpha}
   %\bibliographystyle{abbrv}
   \bibliographystyle{plain}
   %\bibliographystyle{unsrt}   


   \bibliography{dcsplit}
   %\bibliography{swami}
}

% {\scriptsize  is the smallest


==> common_includes.tex <==
% "\includegraphics" command cribs if you have more than one dot(period) in the
% filename. Include the "grffile" package in your document to avoid it. Can
% come in very handy when your image files are auto-generated.
\usepackage{grffile}

% Required to include graphics in the pdf.
\usepackage{graphics,graphicx}

% Math symbols (to get math with different styles like \mathcal, \mathbb)
\usepackage{amsmath,amssymb}

% Require this package to introduce colors in table rows and columns
\usepackage{color, colortbl}

% Table with multiple columns
\usepackage{multicol}

% Advanced macros specification
\usepackage{xparse}

% References
\usepackage{url}
\usepackage{hyperref}

% Automatically figure out the environment
% Note that hyperref has to be loaded before cleveref
% doc: http://ftp.uni-erlangen.de/ctan/macros/latex/contrib/cleveref/cleveref.pdf
\usepackage[noabbrev]{cleveref}
\newcommand{\crefrangeconjunction}{--}

% All things caption and sub-caption related
\usepackage[
  labelfont=footnotesize,
  textfont=footnotesize,
  justification=justified,
  skip=0.5\baselineskip plus 1\baselineskip minus 1\baselineskip
]{subcaption}

\usepackage[
  labelfont={bf,small},
  textfont=small,
  justification=justified,
  skip=0.5\baselineskip plus 1\baselineskip minus 1\baselineskip,
%%   font={stretch=0.85}
]{caption}

\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
\renewcommand\thesubfigure{(\alph{subfigure})}

%% In order to add spaces after macros
\usepackage{xspace}

% Helps in determining size and position of figures
\usepackage{boxedminipage2e}

% Environment to create an algorithm
\usepackage[linesnumbered, lined, boxed]{algorithm2e}
\renewcommand{\listalgorithmcfname}{List of Pseudocode}
\renewcommand{\algorithmcfname}{Pseudocode}
\renewcommand{\algorithmautorefname}{pseudocode}

% Package to include eps figures in \includegraphics. The eps files are
% automatically converted to pdf to be used with pdflatex
\usepackage{epstopdf}

% Tikz -- draw figures in latex.
\usepackage{tikz}
% common tikz packages
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{automata}
\usetikzlibrary{shapes}
\usetikzlibrary{arrows}
\usetikzlibrary{shadows}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.text}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{fit}
\usetikzlibrary{patterns}

% pgf plots are for graphs
\usepackage{pgfplots}
\usepgfplotslibrary{units}

\makeatletter
\tikzset{nomorepostaction/.code=\let\tikz@postactions\pfgutil@empty}
\makeatother



==> envdefs.tex <==
\RequirePackage{enumitem}
\RequirePackage{setspace}
\RequirePackage{xparse}


% A dense itemize environment
\newenvironment{denseitemize}{
\begin{itemize}[noitemsep, topsep=0pt, leftmargin=1.2em]
}{\end{itemize}}

% A dense enumerate environment
\newenvironment{denseenum}{
\begin{enumerate}[noitemsep, topsep=0pt, leftmargin=1.2em]
}{\end{enumerate}}

% A environment for minor headings
\providecommand{\tightcaption}{}%
\renewcommand{\tightcaption}[1]{%
  \begin{spacing}{0.5}
    \caption{#1}
  \end{spacing}
}%

% An environment for inline heading
\providecommand{\inlineheading}{}%
\renewcommand{\inlineheading}[1]{%
  \vspace{1\baselineskip plus 1\baselineskip minus 1\baselineskip} \noindent \textbf{#1:}
}%

% Similar to previous
\providecommand{\minorheading}{}%
\renewcommand{\minorheading}[1]{%
  \vspace{0.5\baselineskip}
  \noindent \textbf{#1}
  \vspace{0.5\baselineskip}
}%

% An environment for writing a custom legend using Tikz
\newenvironment{customlegend}[1][]{%
  \begingroup
  \csname pgfplots@init@cleared@structures\endcsname
  \pgfplotsset{#1}%
}{%
  \csname pgfplots@createlegend\endcsname
  \endgroup
}%

% A command to change the image in the custom legend.
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}

% Use the \S symbol for referencing a section in a concise manner
\providecommand{\secref}{}
\renewcommand{\secref}[1]{\S\ref{#1}}

% Same as above, just another macro name
\providecommand{\xref}{}
\renewcommand{\xref}[1]{\S\ref{#1}}


==> macros.tex <==

% haryadi .. parskip, and parindent
%\setlength\parindent{0pt}
%\setlength\parskip{5pt}

\newcommand{\namen}{DCSplit}
\newcommand{\name}{DCSplit}
%\newcommand{\name}{{\textsc{\small Thumper}}}
%\newcommand{\namen}{{\textsc{Thumper}}}

%\newcommand{\name}{{\textsc{\small DCSplit}}}
\newcommand{\ds}{{\textsc{\small DS}}}
\newcommand{\es}{{\textsc{\small ES}}}
\newcommand{\gtask}{{\textsc{\small GTask}}}
\newcommand{\gtasks}{{\textsc{\small GTasks}}}
\newcommand{\capartition}{{\textsc{\small CAPartition}}}
\newcommand{\capartitions}{{\textsc{\small CAPartitions}}}
 
\newcommand{\beforesec}{\vspace{-.4cm}}
\newcommand{\aftersec}{\vspace{-.3cm}}

\newcommand{\beforesect}{\vspace{-.1cm}}
\newcommand{\aftersect}{\vspace{-.3cm}}

\newcommand{\beforesub}{\vspace{-.3cm}}
\newcommand{\aftersub}{\vspace{-.25cm}}

\newcommand{\beforesubsub}{\vspace{-.2cm}}
\newcommand{\aftersubsub}{\vspace{-.2cm}}

 \newcommand{\zsection}[1]{\section{#1}}
 \newcommand{\zsubsection}[1]{\subsection{#1}}
 \newcommand{\zsubsubsection}[1]{\subsubsection{#1}}

\newcommand{\smush}{0.25in}

\newcommand{\figWidthOne}{3.05in} 
\newcommand{\figWidthHalf}{1.45in} 
\newcommand{\figWidthTwo}{3.05in} 
\newcommand{\figWidthTwop}{1.6in} 
%\newcommand{\figWidthThree}{2.65in} 
\newcommand{\figWidthThree}{2.2in} 
\newcommand{\figWidthSix}{1.1in} 
\newcommand{\figWidthFour}{1.7in} 
\newcommand{\figHeight}{2.0in}
\newcommand{\captionText}[2]{\textbf{#1} \textit{\small{#2}}}

\newcommand{\zbullet}{\hspace{-0.1cm}$\bullet$}

\newcommand{\eg}{e.g.}
\newcommand{\ie}{i.e.}
\newcommand{\etal}{et al.}
\newcommand{\apriori}{\textit{a priori}}

\newcommand{\cut}[1]{}

%-------------------------------------------------------------------
% haryadi -- new command
\newcommand{\msub}[1]{\vspace{1pt}\noindent{\bf #1}}

\newcommand{\ts}[1]{{\tt{\small#1}}}
\newcommand{\tsb}[1]{{\tt{\small{\bf#1}}}}
\newcommand{\tse}[1]{{\tt{\small{\em#1}}}}
\newcommand{\tss}[1]{{\tt{\footnotesize#1}}}
\newcommand{\exc}{$^{\ddag}$}        % except
\newcommand{\EIO}{\ts{EIO}}

%-------------------------------------------------------------------
% For fault injection table
\newcommand{\ip}{bad}
\newcommand{\nullp}{$\emptyset$}

\newcommand{\oops}{o}
\newcommand{\dead}{$\times$}
\newcommand{\alive}{$\surd$}
\newcommand{\unuse}{$\times$}
\newcommand{\use}{$\surd$}
\newcommand{\ic}{$\times$}
\newcommand{\con}{$\surd$}
\newcommand{\gpf}{G}
\newcommand{\npe}{null-pointer}
\newcommand{\usebuta}{$\surd^a$} % unmountable
\newcommand{\hwdetect}{d}

%% TABLE 2
\newcommand{\lateoops}{o$^b$}  % oops happens, but late
\newcommand{\lategpf}{G$^b$}   % gpf, but late
\newcommand{\iop}{i}           % invalid opcode
\newcommand{\detects}{d}       % assertion
\newcommand{\silentret}{s}     % app fails silently
\newcommand{\errorret}{e}      % app returns an error
\newcommand{\appworks}{$\surd$}     % app works!
\newcommand{\usebutar}{$\surd^{ar}$} % read-only and unmountable

\newcommand{\tbls}{\hspace{0.025in}}
\newcommand{\tblss}{\hspace{0.015in}}
\newcommand{\shrinkless}{\vspace{-0.01cm}}

%-------------------------------------------------------------------

%-------------------------------------------------------------------

% axes         
\newcommand{\x}{{\em x}}
\newcommand{\y}{{\em y}}
\newcommand{\xaxis}{x-axis}
\newcommand{\yaxis}{y-axis}

\newcommand{\KB}{~KB}
\newcommand{\KBs}{~KB/s}
\newcommand{\Kbs}{~Kbit/s}
\newcommand{\mbs}{~Mbit/s}
\newcommand{\MB}{~MB}
\newcommand{\GB}{~GB}
\newcommand{\MBs}{~MB/s}
\newcommand{\mus}{\mbox{$\mu s$}}
\newcommand{\ms}{\mbox{$ms$}}


\newcommand{\unix}{{\sc Unix}}
%\newcommand{\NULL}{{\sc NULL}}

\newcommand{\bquote}{\vspace{-0.25cm} \begin{quote}}
\newcommand{\equote}{\end{quote}\vspace{-0.05cm} }

\newcommand{\zquote}[2]{\begin{quote}
#1 --
{\em``#2'' }
%{\bf -- #1 }
\end{quote}}


\newcommand{\XXX}[1]{{\small {\bf (XXX: #1)}}}

\newcommand{\XXXX}{{\bf XXX}}
\newcommand{\xx}{{\bf XXX}}

% normal
\newcommand{\beforecaption}{\begin{spacing}{0.80}}
\newcommand{\aftercaption}{\end{spacing}}
\newcommand{\mycaption}[3]{{\beforecaption\caption{\label{#1}{\bf #2. } {\em \small #3}}\aftercaption}}

\newcommand{\sref}[1]{\S\ref{#1}}

\newcommand{\xxx}[1]{  \underline{ {\small {\bf (XXX: #1)}}}}


\newenvironment{packeditemize}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}


\newcommand{\fwrong}{$\times$}
\newcommand{\smalltt}[1]{\texttt{\fontsize{8.7}{5}\selectfont #1}}
\newcommand{\verysmalltt}[1]{\texttt{\scriptsize #1}}
\newcommand*\rot{\rotatebox{90}}
\newcommand{\toolname}{\mbox{\textsc{\fontsize{9.2}{5}\selectfont Sam}}}
\newcommand{\fstoolname}{\textsc{\fontsize{9.2}{5}\selectfont Bob}}
\newcommand{\Kassandra}{Kassandra}
\newcommand{\microprogram}{microprogram}
\newcommand{\microprograms}{microprograms}
\newcommand{\microinstruction}{microinstruction}
\newcommand{\microinstructions}{microinstructions}
\newcommand{\Microinstructions}{Microinstructions}
\newcommand{\writeSC}{\smalltt{write()}}
\newcommand{\fsyncSC}{\smalltt{fsync()}}
\newcommand{\msyncSC}{\smalltt{msync()}}
\newcommand{\fdatasyncSC}{\smalltt{x fdatasync()}}
\newcommand{\linkSC}{\smalltt{link()}}
\newcommand{\mkdirSC}{\smalltt{mkdir()}}
\newcommand{\fempty}{$\phi$}
\newcommand{\fexists}{$\surd$}
\newcommand{\creatSC}{{\smalltt{creat()}}}
\newcommand{\unlinkSC}{{\smalltt{unlink()}}}
\newcommand{\renameSC}{{\smalltt{rename()}}}

\newcommand{\totbugs}{60}
\newcommand{\totapps}{11}
\newcommand{\totappsw}{eleven}


